Selecting Initial Seeds for Better JVM Fuzzing

Literature in traditional program fuzzing has confirmed that effectiveness is largely impacted by redundancy among initial seeds, thereby proposing a series of seed selection methods. JVM fuzzing, compared to traditional ones, presents unique characteristics, including large-scale and intricate code, and programs with both syntactic and semantic features. However, it remains unclear whether the existing seed selection methods are suitable for JVM fuzzing and whether utilizing program features can enhance effectiveness. To address this, we devise a total of 10 initial seed selection methods, comprising coverage-based, prefuzz-based, and program-feature-based methods. We then conduct an empirical study on three JVM implementations to extensively evaluate the performance of the seed selection methods within two SOTA fuzzing techniques (JavaTailor and VECT). Specifically, we examine performance from three aspects: (i) effectiveness and efficiency using widely studied initial seeds, (ii) effectiveness using the programs in the wild, and (iii) the ability to detect new bugs. Evaluation results first show that the program-feature-based method that utilizes the control flow graph not only has a significantly lower time overhead (i.e., 30s), but also outperforms other methods, achieving 142% to 269% improvement compared to the full set of initial seeds. Second, results reveal that the initial seed selection greatly improves the quality of wild programs and exhibits complementary effectiveness by detecting new behaviors. Third, results demonstrate that given the same testing period, initial seed selection improves the JVM fuzzing techniques by detecting more unknown bugs. Particularly, 21 out of the 25 detected bugs have been confirmed or fixed by developers. This work takes the first look at initial seed selection in JVM fuzzing, confirming its importance in fuzzing effectiveness and efficiency.

==> algorithms/corpus_selection.tex <==
\begin{algorithm}[t]
\small
\KwIn{corpus, k}
\KwOut{corpusSubset}
\SetKwFunction{FMain}{FISS}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{corpus, k}}{
    featureMap $\leftarrow$ new Map\;
    \For{program in corpus}{
        features $\leftarrow$ extractFeatures(program)\;
        featureMap.put(program, features)\;
    }
    sortedList $\leftarrow$ FPS(featureMap)\;
    size $\leftarrow$ sortedList.size() * k / 100\;
    \KwRet sortedList.subList(size)\;
}
\SetKwFunction{FSort}{FPS}
\Fn{\FSort{featureMap}}{
    centroid $\leftarrow$ calCentroid(featureMap)\;
    FP $\leftarrow$ calFarthestPoint(featureMap, centroid)\;
    selectedList $\leftarrow$ FP\;
    selectedMap.put(FP, featureMap.get(FP))\;
    featureMap.remove(FP)\;
    \While{featureMap.size() $\neq$ 0}{
        centroid $\leftarrow$ calCentroid(selectedMap)\;
        FP $\leftarrow$ calFarthestPoint(featureMap, centroid)\;
        selectedList.add(FP)\;
        selectedMap.put(FP, featureMap.get(FP))\;
        featureMap.remove(FP)\;
    }
    \KwRet selectedList\;
}
\caption{Initial seed selection process of \feabase{}}
\label{algo:corpusreduction}
\end{algorithm}


==> comments.tex <==
\usepackage{datenumber}

\def\mybar#1{%%
  #1s & {\color{grey}\rule{#1cm}{8pt}}}

\newcommand\revdif[2]{\nb{#1}{\color{orange}#2}}
\newcommand\rev[2]{\nb{#1}{\color{red}#2}}
\newcommand{\nb}[2]{
	{
		{\color{red}{
				\fbox{\bfseries\sffamily\scriptsize#1}
				{\sffamily$\triangleright~${\it\sffamily #2}$~\triangleleft$}
	}}}
}


\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36}


\newcommand\respond[2]{{\nb{#2}{\color{blue}#1}}}

\newcommand{\impacttext}[1]{{\color{red}#1}}
\newcommand{\rone}[1]{\colorbox{yellow}{\textbf{[#1]}}}
\newcommand\revise[1]{\nb{Revised}{\color{orange}#1}}
\newcommand\wang[1]{\nb{Wang}{\color{red}#1}}
\newcommand\chen[1]{\nb{Chen}{\color{magenta}#1}}
\newcommand\gao[1]{\nb{Gao}{\color{violet}#1}}
\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME] #1}}\xspace}
\newcommand{\cn}{{\color{violet}[citation required]}}
\newcommand{\tbd}{{\color{green}[To Be Done!]}}

\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36}

%%% Date configs
% \newcounter{dateone}
% \newcounter{datetwo}

% \newcommand{\difftoday}[3]{%
%       \setmydatenumber{dateone}{\the\year}{\the\month}{\the\day}%
%       \setmydatenumber{datetwo}{#1}{#2}{#3}%
%       \addtocounter{datetwo}{-\thedateone}%
%       \the\numexpr-\thedatetwo/365\relax\space year(s),
%       \the\numexpr(-\thedatetwo - (-\thedatetwo/365)*365)/30\relax\space month(s)
% } 

\newcounter{dateone}\newcounter{datetwo}%
\newcommand{\daydifftoday}[3]{%
\setmydatenumber{dateone}{\the\year}{\the\month}{\the\day}%
\setmydatenumber{datetwo}{#1}{#2}{#3}%
\addtocounter{datetwo}{-\thedateone}%
\thedatetwo
}


==> tables/dtjvms.tex <==
\begin{table}[]
\caption{Differential testing JVM versions}
\label{tab:dtjvms}
\centering
\small
\setlength{\tabcolsep}{3.5mm}
\renewcommand{\arraystretch}{1.5}
\begin{spacing}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccr}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}OpenJDK\\ Version\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}JVM\\ Implementation\end{tabular}} &
  \multicolumn{1}{c}{\textbf{ Version}} \\ \midrule
\multirow{6}{*}{OpenJDK8}  & \multirow{2}{*}{HotSpot}     &  \cellcolor[HTML]{E8E8E8}build 25.0-b70    \\ \cline{3-3} 
                           &                              & build 25.345-b01                             \\ \cmidrule(l){2-3} 
                           & \multirow{2}{*}{OpenJ9}      & \cellcolor[HTML]{E8E8E8}build openj9-0.8.0     \\ \cline{3-3} 
                           &                              & build openj9-0.32.0                             \\ \cmidrule(l){2-3} 
                           & \multirow{2}{*}{Bisheng JDK} & \cellcolor[HTML]{E8E8E8}build 25.302-b13     \\ \cline{3-3} 
                           &                              & build 25.332-b11                             \\ 
                           \hline
\multirow{6}{*}{OpenJDK11}  & \multirow{2}{*}{HotSpot}     &  \cellcolor[HTML]{E8E8E8}build 11+28    \\ \cline{3-3} 
                           &                              & build 11.0.16+8                             \\ \cmidrule(l){2-3} 
                           & \multirow{2}{*}{OpenJ9}      & \cellcolor[HTML]{E8E8E8}build openj9-0.12.0     \\ \cline{3-3} 
                           &                              & build openj9-0.32.0                             \\ \cmidrule(l){2-3} 
                           & \multirow{2}{*}{Bisheng JDK} & \cellcolor[HTML]{E8E8E8}build 11.0.12+13     \\ \cline{3-3} 
                           &                              & build 11.0.15+11                             \\ 
                           \hline
\multicolumn{3}{l}{Shadow represents the used old build of the corresponding JVM.}
\end{tabular}
}
\end{spacing}
\end{table}

==> tables/old_inconsistencies.tex <==
\begin{table*}[htbp]
\caption{Comparison results of different methods in terms of the number of unique inconsistencies}
\label{tab:unique_inconsistency}
\begin{spacing}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{rcccccccccccccccccc}
\toprule

\multicolumn{1}{c}{\multirow{3}{*}{Method}} & 
    \multicolumn{6}{|c}{P1 (RQ1)} & 
    \multicolumn{6}{|c}{P2 (RQ1)} & 
    \multicolumn{6}{|c}{P3 (RQ2)}   \\ 
\cmidrule(l){2-19}

\multicolumn{1}{c}{} &
    \multicolumn{3}{|c}{JavaTailor} &
    \multicolumn{3}{|c}{VECT} &
    \multicolumn{3}{|c}{JavaTailor} &
    \multicolumn{3}{|c}{VECT} &
    \multicolumn{3}{|c}{JavaTailor} &
    \multicolumn{3}{|c}{VECT} \\
\cmidrule(l){2-19}
  
\multicolumn{1}{c}{} &
    \multicolumn{1}{|c}{20\%} &
    \multicolumn{1}{c}{35\%} &
    \multicolumn{1}{c}{50\%} &
    \multicolumn{1}{|c}{20\%} &
    \multicolumn{1}{c}{35\%} &
    \multicolumn{1}{c}{50\%} &
    \multicolumn{1}{|c}{20\%} &
    \multicolumn{1}{c}{35\%} &
    \multicolumn{1}{c}{50\%} &
    \multicolumn{1}{|c}{20\%} &
    \multicolumn{1}{c}{35\%} &
    \multicolumn{1}{c}{50\%} &
    \multicolumn{1}{|c}{20\%} &
    \multicolumn{1}{c}{35\%} &
    \multicolumn{1}{c}{50\%} &
    \multicolumn{1}{|c}{20\%} &
    \multicolumn{1}{c}{35\%} &
    \multicolumn{1}{c}{50\%}  \\
\midrule

\multicolumn{1}{l}{\fullset{}}  & 
    \multicolumn{3}{|c}{5.4} & 
    \multicolumn{3}{|c}{9.0} & 
    \multicolumn{3}{|c}{6.4} & 
    \multicolumn{3}{|c}{7.8} & 
    \multicolumn{3}{|c}{5.0} & 
    \multicolumn{3}{|c}{4.8} \\
    \midrule

\multicolumn{1}{l}{\randomset{}} & 
    \multicolumn{1}{|c}{5.0} & 
    \multicolumn{1}{c}{4.6} & 
    \multicolumn{1}{c}{5.4} & 
    
    \multicolumn{1}{|c}{5.6} & 
    \multicolumn{1}{c}{6.2} & 
    \multicolumn{1}{c}{7.4} & 
    
    \multicolumn{1}{|c}{6.2} & 
    \multicolumn{1}{c}{\textbf{7.4}} & 
    \multicolumn{1}{c}{5.8} & 
    
    \multicolumn{1}{|c}{4.0} & 
    \multicolumn{1}{c}{5.0} & 
    \multicolumn{1}{c}{5.4} & 
    
    \multicolumn{1}{|c}{\textbf{5.2}} & 
    \multicolumn{1}{c}{4.4} & 
    \multicolumn{1}{c}{\textbf{5.6}} & 
    
    \multicolumn{1}{|c}{4.0} & 
    \multicolumn{1}{c}{3.8} & 
    \multicolumn{1}{c}{4.2} \\  \midrule
    
\multicolumn{1}{l}{\minset{}} & 
    \multicolumn{1}{|c}{\textbf{7.4}} & 
    \multicolumn{1}{c}{\textbf{6.0}} & 
    \multicolumn{1}{c}{\textbf{7.8}} & 
    
    \multicolumn{1}{|c}{7.2} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{9.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}8.4} & 

    \multicolumn{1}{|c}{\textbf{8.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{8.2}} & 
    \multicolumn{1}{c}{\textbf{8.6}} & 
    
    \multicolumn{1}{|c}{\textbf{9.2}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{8.6}} & 
    \multicolumn{1}{c}{\textbf{9.2}} & 

    \multicolumn{1}{|c}{5.0} & 
    \multicolumn{1}{c}{\textbf{5.2}} & 
    \multicolumn{1}{c}{4.8} & 
    
    \multicolumn{1}{|c}{3.8} & 
    \multicolumn{1}{c}{4.8} & 
    \multicolumn{1}{c}{4.4} \\ 
    
\multicolumn{1}{l}{\peachset{}} & 
    \multicolumn{1}{|c}{5.0} & 
    \multicolumn{1}{c}{5.2} & 
    \multicolumn{1}{c}{\textbf{6.4}} & 
    
    \multicolumn{1}{|c}{5.4} & 
    \multicolumn{1}{c}{6.6} & 
    \multicolumn{1}{c}{7.4} & 

    \multicolumn{1}{|c}{\cellcolor[HTML]{DDDDDD}\textbf{9.2}} & 
    \multicolumn{1}{c}{\textbf{7.4}} & 
    \multicolumn{1}{c}{\textbf{7.8}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{DDDDDD}\textbf{9.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{9.4}} & 
    \multicolumn{1}{c}{\textbf{9.2}} & 

    \multicolumn{1}{|c}{4.2} & 
    \multicolumn{1}{c}{4.6} & 
    \multicolumn{1}{c}{4.4} & 
    
    \multicolumn{1}{|c}{3.6} & 
    \multicolumn{1}{c}{\textbf{5.2}} & 
    \multicolumn{1}{c}{3.8} \\ \midrule
\multicolumn{1}{l}{\hotset{}} & 
    \multicolumn{1}{|c}{\textbf{6.4}} & 
    \multicolumn{1}{c}{\textbf{7.2}} & 
    \multicolumn{1}{c}{\textbf{8.0}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{CCCCCC}\textbf{9.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}8.6} & 
    \multicolumn{1}{c}{7.8} & 

    \multicolumn{1}{|c}{\textbf{7.8}} & 
    \multicolumn{1}{c}{\textbf{7.2}} & 
    \multicolumn{1}{c}{\textbf{7.8}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{CCCCCC}\textbf{9.6}} & 
    \multicolumn{1}{c}{\textbf{8.0}} & 
    \multicolumn{1}{c}{7.4} & 

    \multicolumn{1}{|c}{\textbf{7.6}} & 
    \multicolumn{1}{c}{\textbf{5.8}} & 
    \multicolumn{1}{c}{\textbf{5.4}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{DDDDDD}\textbf{6.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{7.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{7.6}} \\ 
\midrule
\multicolumn{1}{l}{\tfidfset{}} & 
    \multicolumn{1}{|c}{\textbf{7.2}} & 
    \multicolumn{1}{c}{\textbf{8.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{9.6}} & 
    
    \multicolumn{1}{|c}{6.6} & 
    \multicolumn{1}{c}{7.6} & 
    \multicolumn{1}{c}{7.6} & 

    \multicolumn{1}{|c}{\textbf{7.0}} & 
    \multicolumn{1}{c}{\textbf{7.2}} & 
    \multicolumn{1}{c}{\textbf{6.8}} & 
    
    \multicolumn{1}{|c}{6.4} & 
    \multicolumn{1}{c}{6.0} & 
    \multicolumn{1}{c}{5.6} & 

    \multicolumn{1}{|c}{\textbf{6.8}} & 
    \multicolumn{1}{c}{\textbf{5.6}} & 
    \multicolumn{1}{c}{\textbf{6.8}} & 
    
    \multicolumn{1}{|c}{4.8} & 
    \multicolumn{1}{c}{\textbf{5.2}} & 
    \multicolumn{1}{c}{\textbf{6.8}} \\ 
\multicolumn{1}{l}{\astset{}} & 
    \multicolumn{1}{|c}{\cellcolor[HTML]{CCCCCC}\textbf{8.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{9.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{9.4}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{DDDDDD}8.6} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}8.6} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{10.0}} & 

    \multicolumn{1}{|c}{\cellcolor[HTML]{CCCCCC}\textbf{11.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{9.2}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{11.6}} & 
    
    \multicolumn{1}{|c}{\textbf{9.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{9.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{10.2}} & 

    \multicolumn{1}{|c}{\textbf{6.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{7.8}} & 
    \multicolumn{1}{c}{\textbf{7.0}} & 
    
    \multicolumn{1}{|c}{\textbf{6.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{6.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{7.0}} \\ 
\multicolumn{1}{l}{\cfgset{}} & 
    \multicolumn{1}{|c}{\cellcolor[HTML]{BBBBBB}\textbf{12.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{13.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{12.0}} &
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{BBBBBB}\textbf{12.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{14.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{16.2}} & 

    \multicolumn{1}{|c}{\cellcolor[HTML]{BBBBBB}\textbf{15.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{15.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{17.2}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{BBBBBB}\textbf{16.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{16.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{15.4}} & 

    \multicolumn{1}{|c}{\cellcolor[HTML]{CCCCCC}\textbf{8.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{7.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{10.4}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{CCCCCC}\textbf{7.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{6.6}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{9.6}} \\ 
\midrule
\multicolumn{1}{l}{\codebertset{}} & 
    \multicolumn{1}{|c}{\textbf{7.6}} & 
    \multicolumn{1}{c}{\textbf{7.0}} & 
    \multicolumn{1}{c}{\textbf{8.6}} &  
    
    \multicolumn{1}{|c}{6.2} & 
    \multicolumn{1}{c}{7.4} & 
    \multicolumn{1}{c}{8.2} & 
    
    \multicolumn{1}{|c}{\textbf{6.6}} & 
    \multicolumn{1}{c}{\textbf{7.6}} & 
    \multicolumn{1}{c}{\textbf{8.2}} & 
    
    \multicolumn{1}{|c}{6.6} & 
    \multicolumn{1}{c}{6.8} & 
    \multicolumn{1}{c}{\textbf{8.8}} & 

    \multicolumn{1}{|c}{\cellcolor[HTML]{DDDDDD}\textbf{7.8}} & 
    \multicolumn{1}{c}{\textbf{7.0}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{7.6}} &

    \multicolumn{1}{|c}{\textbf{6.2}} & 
    \multicolumn{1}{c}{\textbf{6.0}} & 
    \multicolumn{1}{c}{\textbf{6.2}} \\ 
\multicolumn{1}{l}{\infercodeset{}} & 
    \multicolumn{1}{|c}{\textbf{7.2}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{8.8}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{9.4}} &
    
    \multicolumn{1}{|c}{7.8} & 
    \multicolumn{1}{c}{7.8} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}8.4} & 

    \multicolumn{1}{|c}{6.4} & 
    \multicolumn{1}{c}{\textbf{7.8}} & 
    \multicolumn{1}{c}{\textbf{6.6}} & 
    
    \multicolumn{1}{|c}{7.2} & 
    \multicolumn{1}{c}{5.4} & 
    \multicolumn{1}{c}{5.6} & 

    \multicolumn{1}{|c}{\cellcolor[HTML]{BBBBBB}\textbf{10.2}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{8.8}} & 
    \multicolumn{1}{c}{\textbf{7.4}} & 
    
    \multicolumn{1}{|c}{\cellcolor[HTML]{BBBBBB}\textbf{9.2}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{BBBBBB}\textbf{8.0}} & 
    \multicolumn{1}{c}{4.2} \\ 
\multicolumn{1}{l}{\plbartset{}} & 
    \multicolumn{1}{|c}{\textbf{7.4}} & 
    \multicolumn{1}{c}{\textbf{8.2}} & 
    \multicolumn{1}{c}{\textbf{8.0}} & 
    
    \multicolumn{1}{|c}{7.6} & 
    \multicolumn{1}{c}{7.8} & 
    \multicolumn{1}{c}{7.2} & 

    \multicolumn{1}{|c}{6.2} & 
    \multicolumn{1}{c}{\textbf{7.0}} & 
    \multicolumn{1}{c}{\textbf{6.6}} & 
    
    \multicolumn{1}{|c}{6.2} & 
    \multicolumn{1}{c}{5.6} & 
    \multicolumn{1}{c}{5.4} & 

    \multicolumn{1}{|c}{\textbf{6.2}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{7.4}} & 
    \multicolumn{1}{c}{4.8} & 
    
    \multicolumn{1}{|c}{3.6} & 
    \multicolumn{1}{c}{3.8} & 
    \multicolumn{1}{c}{2.4} \\ 
\multicolumn{1}{l}{\codetset{}} & 
    \multicolumn{1}{|c}{\cellcolor[HTML]{DDDDDD}\textbf{8.0}} & 
    \multicolumn{1}{c}{\textbf{8.0}} & 
    \multicolumn{1}{c}{\textbf{9.0}} &  
    
    \multicolumn{1}{|c}{7.2} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}8.6} & 
    \multicolumn{1}{c}{8.2} & 

    \multicolumn{1}{|c}{6.4} & 
    \multicolumn{1}{c}{\textbf{7.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{8.8}} & 
    
    \multicolumn{1}{|c}{6.6} & 
    \multicolumn{1}{c}{\textbf{8.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{DDDDDD}\textbf{9.6}} & 

    \multicolumn{1}{|c}{\textbf{5.4}} & 
    \multicolumn{1}{c}{\textbf{6.4}} & 
    \multicolumn{1}{c}{\cellcolor[HTML]{CCCCCC}\textbf{7.8}} &
    
    \multicolumn{1}{|c}{\textbf{6.2}} & 
    \multicolumn{1}{c}{\textbf{5.6}} & 
    \multicolumn{1}{c}{\textbf{6.4}} \\ 
    
\bottomrule
\end{tabular}
}
\vspace{-.5cm}
\end{spacing}
\end{table*}
